A Lightweight Modular Continuum Manipulator with IMU-based Force Estimation

Most aerial manipulators use serial rigid-link designs, which results in large forces when initiating contacts during manipulation and could cause flight stability difficulty. This limitation could potentially be improved by the compliance of continuum manipulators. To achieve this goal, we present the novel design of a compact, lightweight, and modular cable-driven continuum manipulator for aerial drones. We then derive a complete modeling framework for its kinematics, statics, and stiffness (compliance). The modeling framework can guide the control and design problems to integrate the manipulator to aerial drones. In addition, thanks to the derived stiffness (compliance) matrix, and using a low-cost IMU sensor to capture deformation angles, we present a simple method to estimate manipulation force at the tip of the manipulator. We report preliminary experimental validations of the hardware prototype, providing insights on its manipulation feasibility. We also report preliminary results of the IMU-based force estimation method.

==> content/acknowledgement.tex <==
\begin{acknowledgment}
This research was supported in part by USDA-NIFA Grant No. 2021-67022-35977. \par
%
\end{acknowledgment}

==> content/discussion.tex <==
\section{Discussion}

Aerial manipulation is getting increasing attention in recent years. The integration of robotic arms and aerial vehicle platforms leads to a broad range of potential applications. 
The essential goal of aerial manipulation is its accessibility of operating at a high altitude indoor or outdoor workspace that cannot be easily reached by human workers, at the same time to reduce cost and time. Some potential applications include the inspection and maintenance of power lines, the transportation of objects, and disaster assistance and rescue. All of these applications require the UAVs to have some physical interactions with the environment and/or human, to operate for a relatively long period of time, to manipulate tools, and to transport goods. 
For the purpose of this proposed aerial continuum arm design and prototype, researchers plan to focus on grasping and perching tasks moving forward, which are the basic functionalities needed by the aforementioned applications. The use of a continuum arm helps improve robustness and also provides a high tolerance in UAV's pose accuracy. Researchers also aim to add a gripper at the tip of the continuum arm to complete the aerial manipulator system for more advanced kinematic and dynamic analysis and overall experiments. In addition, further investigation on how the continuum arm mechanical design impacts the performance of the aerial manipulator system is needed.\par

Currently, aerial manipulation activities are tightly limited by aviation administration regulations all over the world. UAVs with certain weight limits must fly in permitted airspaces by certified remote pilots under good weather visibility and within visual line-of-sight. It is the researchers responsibility to know the UAV's rules and regulations and to design experiments with those in mind. \par

